Security Assurance Cases for Road Vehicles: an Industry Perspective

Assurance cases are structured arguments that are commonly used to reason about the safety of a product or service. Currently, there is an ongoing push towards using assurance cases for also cybersecurity, especially in safety-critical domains, like automotive. While the industry is faced with the challenge of defining a sound methodology to build security assurance cases, the state of the art is rather immature. Therefore, we have conducted a thorough investigation of the (external) constraints and (internal) needs that security assurance cases have to satisfy in the context of the automotive industry. This has been done in the context of two large automotive companies in Sweden. The end result is a set of recommendations that automotive companies can apply in order to define security assurance cases that are (i) aligned with the constraints imposed by the existing and upcoming standards and regulations and (ii)harmonized with the internal product development processes and organizational practices. We expect the results to be also of interest for product companies in other safety-critical domains, like healthcare, transportation, and so on

==> breakout.tex <==
The usage scenarios selected for the break-out session were US3, US6, and US12.


\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Compliance with the company's cybersecurity standard 
			\\ \midrule
			                      Who& Owner: Project manager
			                      \\ & For: Product Owner
			                      \\ & Contributors: Project team, train
			                      \\& QA: Verification team
			                      \\& Maintenance: Line organization
			  \\ \midrule
			                      When&Start: Early project phase
			                      \\ &Evolves: Change related
			                      \\ & Changes: Wrong assumptions, change requests, bugs.
			                      \\ &Finish: Release gate
			\\ \midrule
			                      How&Evidence: Risk assessments verification reports, review reports.
			\\ \midrule
			                      Challenges& Dependencies and support                      
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US3}
		\label{res_bo_1}
	\end{center}
\end{table}

\paragraph{US3} Table \ref{res_bo_1} shows the answers provided by the team which worked on US3. The participants decided that the scope of the case from this US is the same as an internal project's scope. This was then used to answer the questions in the exercise. The only claim suggested by the team is a high level one for complying with the company's security standard. When it comes to the roles, the participants suggested that the project manager should be the owner of the case, and that the project team would contribute towards creating and verifying it. The case should be then handed to the owner of the product in which the project took place for integrating it with the product's case. The life-cycle of the case starts in an early phase of the project as per the team. However, they did not specify a particular phase. The case then evolves as the project evolves, and finishes when the project is released, after it serves its main goal in the decision making of releasing the project. The team suggest multiple sources for evidence, such as risk assessment, review, and verification reports. The main challenge pointed out by the team are managing and tracing dependencies between the claims of this case and claims of other projects, as well as the claims of the product's case. A second challenge is to provide the support needed to work with security assurance cases, both when it comes to competences and tools.

\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Following standards and industry best practices
			                      \\& Legal compliance, e.g., GDPR
			                      \\& Fulfillment of security attributes
			\\ \midrule
			                      Who& Owner: Product owner
			                      \\ & Contributors: product team, security team
			                      \\& QA: Product owner
			                      \\& Maintenance: Product owner
			  \\ \midrule
			                      When&Start: Concept study phase
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US6}
		\label{res_bo_2}
	\end{center}
\end{table}

\paragraph{US6} Table \ref{res_bo_2} shows the answers provided by the team which worked on US6. The team members were not able to set a clear scope of the case of this US as it depends heavily on the product in question. Hence, it was difficult for them to answer many of the questions in the exercise. The main claims suggested by the team were about complying with standards and regulations, as well as the fulfillment of security attributes, such as confidentiality, integrity, and availability. When it comes to the \emph{who} question, the team had a very hard time finding out who the tasks associated with SAC should be assigned to. At the end, they decided that the product owner for which the SAC is created, should also own the SAC, be responsible of its quality assurance, and maintenance. Other contributors according to the team are the product team for creating the case, and the security team for support. The last question partially answered by the team was the \emph{when} question, and the suggestion was to start building the SAC in a very early stage at the product development phase, namely the concept study phase. However, the team did not discuss creating SAC for an existing product.

\begin{table}
	\begin{center}
		\begin{tabular}{p{2cm}p{6cm}}

		
			\\       \textbf{Question}
	        & \textbf{Answer}

			\\ \midrule
			                      What&Claims that sufficient measures have been taken
			\\ \midrule
			                      Who& Owner: Lawyer, task manager, investigation leader.
			                      \\ & For: Upper management, court
			                      \\ & Contributors: SMEs, product owner
			                      \\& QA: Lawyers, external security experts
			                      \\& Maintenance: Product owner
			  \\ \midrule
			                      When&Start: At start of court case ( assuming that the SAC is already created for a certain project or product)
			                      \\ &Evolves: As evidence are being collected
			                      \\ & Changes: As evidence are being added.
			                      \\ &Finish: When the court case is closed
			\\ \midrule
			                      How&Evidence: TARA, verification and validation reports, and risk mitigation documentation
			\\ \midrule
			                      Challenges&Traceability needs to be improved (for the documents used in SAC)
			                      \\&Roles and ownership identification
			\\ \bottomrule
		\end{tabular}
		\caption{Summary of the discussion in the break-out session about US12}
		\label{res_bo_3}
	\end{center}
\end{table}

\paragraph{US12} Table \ref{res_bo_3} shows the the results of the break out session's exercise for US12. The participants considered the SAC related to this US to be limited to the legal case. This means that the SAC would be created (or extracted fro another SAC) only when needed. This is when a legal case is filed against the company for security related issues. The main goal of this SAC is showing that sufficient security measures have been taken for the system / component in question, according to the participants. When it comes to the roles, the participants suggested multiple owners for the SAC, e.g., the lawyer responsible for the legal case, or investigation leader. The creation of the SAC would be contributed by the product owner and the Subject Matter Experts of the product in question, and the quality assurance would be the responsibility of the users of the case, i.e., the lawyers, with help from external security experts. When it comes to maintaining the SAC, the team suggested that the product owner should take on that task, as it would be a part of a generic one for the product. The life-cycle of this SAC according to the team follows the life-cycle of the legal case, meaning that the SAC is created at the start of the legal case, evolves as the legal case evolves, and finishes when the legal case is closed. The participants also suggested evidence for the SAC, e.g., Threat Analysis and Risk Assessment (TARA) reports, verification results, and risk mitigation documents. The team considered traceability for the relevant documents of the SAC to be a major challenge in addition to organisational challenges in identifying the right roles for SAC related tasks.

TODO: summary, etc...

To summarize, we got th
It is clear that even though we got answers on questions, we still needed to dig deeper into the US as in many cases, the participants were not confident in their answers. For example in US12, the team answered all the who questions, but still mentioned a challenge to identify the roles when SAC will be applied in the company. 
